Wasserstein-based fairness interpretability framework for machine learning models

The objective of this article is to introduce a fairness interpretability framework for measuring and explaining the bias in classification and regression models at the level of a distribution. In our work, we measure the model bias across sub-population distributions in the model output using the Wasserstein metric. To properly quantify the contributions of predictors, we take into account the favorability of both the model and predictors with respect to the non-protected class. The quantification is accomplished by the use of transport theory, which gives rise to the decomposition of the model bias and bias explanations to positive and negative contributions. To gain more insight into the role of favorability and allow for additivity of bias explanations, we adapt techniques from cooperative game theory.

==> declarations.tex <==
\section*{Declarations}\label{sec::declarations}

\subsection*{Funding}
Not applicable.

\subsection*{Conflicts of interest/Competing interests}
Not applicable.

\subsection*{Ethics approval}
Not applicable.

\subsection*{Consent to participate}
Not applicable.

\subsection*{Consent for publication}
Not applicable.

\subsection*{Availability of data and material}
All data in the examples of the article are synthetic, except for the dataset used in Section 5.3 which was taken from the UCI Machine Learning Repository which can be found at \url{https://archive.ics.uci.edu/ml/datasets/census+income}. In the synthetic examples, we provide explicit formulas for the joint data distribution.


\subsection*{Code availability}

Algorithm 1 in Section 5.3 presents the steps on the application of our interpretability framework. Since the code of Algorithm 1 is the intellectual property of Discover Financial Services, we provide the list of publicly available Python packages for its implementation. We used the package \texttt{sklearn.ensemble} for model training, \texttt{numpy.random} for generating random parameters and the joint distribution of synthetic data, \texttt{sklearn.metrics} for  computing performance metrics, \texttt{empirical\_distribution.ECDF} from the package \texttt{statsmodels.distributions} for computing the Wasserstein distance, and for the computation of Shapley values we used \texttt{itertools.combinations} and \texttt{numpy}.

\subsection{Authors' contributions}
Not applicable.
